Physics at the e+ e- Linear Collider

A comprehensive review of physics at an e+e- Linear Collider in the energy range of sqrt{s}=92 GeV--3 TeV is presented in view of recent and expected LHC results, experiments from low energy as well as astroparticle physics.The report focuses in particular on Higgs boson, Top quark and electroweak precision physics, but also discusses several models of beyond the Standard Model physics such as Supersymmetry, little Higgs models and extra gauge bosons. The connection to cosmology has been analyzed as well.

==> Astro/epjrev_astrocosrel.tex <==
\section{Connection to astroparticle physics and cosmology }
\label{astro}
%Your text comes here. 
%Text with citations \cite{Belanger:2012jn} and \cite{Olive:2012ck}.

\subsection{Introduction}
\label{sec:astro1}

While an enormous amount of energy is spent on the search for physics
beyond the standard model, perhaps the most compelling reason for
expecting physics beyond the standard model is dark matter. The evidence
for dark matter is overwhelming.  On galactic scales, one observes
relatively flat rotation curves \cite{rot} which can not be accounted
for by the observed luminous component of the galaxy.  The simplest
interpretation of these observations are that nearly all spiral galaxies
are embedded in a large galactic halo of dark matter which lead to
rather constant rotational velocities at large distances from the center
of the galaxy.  X-ray emission from hot gas surrounding large elliptical
galaxies and clusters of galaxies also require a large potential well
(to gravitationally bind the hot gas) which can not be accounted for by
the galaxy or gas itself \cite{xray}.  Gravitational lensing also
implies large gravitational potentials from unseen matter on the scale
of clusters of galaxies \cite{lense}.  In addition, there are
observations of both x-ray emitting hot gas and gravitational lensing in
the same systems \cite{both} which all point to the presence of dark
matter.

On larger, scales, baryon acoustic oscillations \cite{bao} indicate a
matter component $\Omega_m = \rho_m/\rho_c \simeq 0.25$, where $\rho_c =
1.88 \times 10^{-29} g cm^{-3}$ is the critical energy density for
spatial flatness. However, the baryon density of the universe from big
bang nucleosynthesis (BBN) \cite{bbn} is restricted to $\Omega_B h^2
\alst 0.03$ where $h = 0.71$ is the Hubble parameter in units of 100
km/s/Mpc. Furthermore, both the estimate from baryon acoustic
oscillations and nucleosynthesis are in complete agreement with the
determination of both the total matter density and baryon density from
the cosmic microwave background anisotropy spectrum \cite{wmap} which
yields a dark matter density of \be \Omega h^2 = 0.111 \pm 0.006
\label{wmapden} \ee

As we will see, there are no candidates for the dark matter of the
Universe found in the Standard Model. Thus the body of evidence for dark
matter clearly points to physics beyond the Standard Model.  Below, we
will briefly describe some of the well-studied candidates for dark
matter with an emphasis on their relevance for a future LC.

\subsection{Candidates}
\label{s:cand}

With the putative discovery of the Higgs boson, 
the Standard Model field content is complete.
As dark matter stable of long lived, there are only two 
possible a priori candidates for dark matter in the Standard Model.
While baryonic dark matter may account for some of the dark matter
in galactic halos, it can not make up the bulk of the dark matter in the Universe.
As noted above, BBN limits the baryon density to less than 25\% of the total
amount of non-relativistic matter in the universe, which is consistent with the
determination of the baryon density from microwave background anisotropies.
However,  a dominant component of 
baryonic dark matter  even on the galactic scale is problematic \cite{Hegyi:1985yu}.
Put simply, baryons tend to clump and form stellar-like objects.
While massive objects such as white dwarfs or neutron stars or black holes may be dark,
they are typically associated with heavy element production and a significant number
of these objects would produce excessive metallicity. 
Smaller jupiter-like objects would require a very special
mass distribution to avoid constraints from luminosity density in the red and infrared.
More concrete constraints are obtained from microlensing observations \cite{pac}
where the contribution of such objects (collectively known as MACHOs) is 
limited to less than 25\% of the halo for masses   $2 \times 10^{-7} M_\odot < M < 1
M_\odot$.

Another potential possibility for a dark matter candidate in the standard model
is a neutrino. Indeed, neutrino oscillation experiments
indicate that at least one neutrino has a mass in excess of 0.05 eV. 
This would correspond to a cosmological contribution, $\Omega_\nu h^2 > 5\times 10^{-4}$.
However there are upper limits to the sum of neutrino masses from
large scale structure considerations.
In particular, using the 7-year WMAP data and including observations from
SDSS and HST, one finds that the sum of neutrino masses is constrained to be
$\sum m_\nu < 0.44$ eV corresponding to $\Omega_\nu h^2 < 4.5 \times 10^{-3}$
\cite{Hannestad:2010yi}.

At this time, if there is any firm indication of physics beyond the standard model,
it comes from our understanding of dark matter in the Universe.
While not all dark matter candidates can be probed by a future
linear collider, we are will restrict our attention to those that can.
Thus we will not discuss the possibility of sterile neutrinos or axions below
and we concentrate on those candidates with potential signatures at the LC.





\subsubsection{Supersymmetric Candidates}

The supersymmetric extension of the Standard Model
is one of the most studied example of physics beyond the Standard Model
and is currently being tested at the LHC. Its motivations (which we will not review here)
include the stabilization of the weak scale hierarchy, gauge coupling unification,
radiative electroweak symmetry breaking, and the prediction of a light Higgs boson
($m_h \alst 130$ GeV) which has probably been borne out by experiment \cite{lhch}.
In models with R-parity conservation, another prediction of supersymmetric
models, is the existence of one stable particle, which if neutral, may be candidate 
for the dark matter. This is the lightest supersymmetric particle of LSP.  
Below, we review some of the most studied 
realizations of the low energy supersymmetry.

For the most part, we will restrict our attention here to the minimal supersymmetric
standard model (MSSM) (though see below for a discussion of the next to 
minimal model or NMSSM). The minimal model is defined
by the superpotential 
\be
W =  \bigl( y_e H_1 L e^c + y_d H_1 Q d^c + y_u H_2 Q u^c \bigr) +  \mu H_1 H_2 ,
\label{WMSSM}
\ee
Beyond the parameters assoicated with the Standard Model, the
superpotenital introduces a mixing term between the two Higgs doublets in the MSSM.
The bulk of the new parameters are associated with supersymmetry breaking
and are associated with soft scalar masses, gaugino masses, and so-called 
bi- and tri-linear terms, $B$ and $A$. There are well over 100 new parameters
in the minimal theory and we are thus forced to make some (well motivated)
simplifications as we discuss below. 


\paragraph{The CMSSM}

As is clear, supersymmetry must be broken, and one way of transmitting 
the breaking of supersymmetry to the low energy sector of the theory is through
gravity.  Indeed the extension of global supersymmetry to supergravity
is in some sense necessary to ensure the (near) vanishing of the
cosmological constant in models with weak scale supersymmetry breaking.
Gravity mediated supersymmetry breaking impose a number of boundary conditions
on the supersymmetry breaking masses at some high energy renormalization scale,
which is usually taken to be the same scale at which gauge coupling unification occurs, $M_{GUT}$.
In gravity mediated models, one often finds that all scalar masses are equal at $M_{GUT}$
defining a universal scalar mass $m_0$. Similarly, all gaugino mass and trilinear terms
are also universal at $M_{GUT}$, with values $m_{1/2}$ and $A_0$ respectively.

In these gravity mediated supersymmetry breaking models,
supersymmetry breaking masses and gauge and Yukawa couplings are
are run down from the universality scale and often trigger electraoweak symmetry
breaking as one or both of the soft Higgs masses, $m_{1,2}^2$ run negative.
In true minimal supergravity models or mSUGRA, the scalar mass is 
equal to the gravitino mass, $m_0 = m_{3/2}$, and the $B$-term is given
by $B_0 = A_0 - m_0$.  One consequence of the latter relation
is the determination of the two Higgs vacuum expectation values
as the soft masses are run down to the weak scale. Since
one combination of the two vevs determines the $Z$ gauge boson mass, it is common
to choose the two vev's as input parameters (the other combination is the ratio of 
vevs and defined as $\tan \beta = v_2/v_1$) and discard the relation between $B_0$
and $A_0$. Instead both $B$ and $\mu$ can be calculated at the weak from $M_Z$ and $\tan \beta$.
If the relation between the gravitino mass and $m_0$, is also dropped, we have 
the constrained version of the MSSM known as the CMSSM.

The CMSSM is therefore a four parameter theory (the sign of $\mu$ must also be specified).
For given values of $\tan \beta$, $A_0$,  and $sgn(\mu)$, the regions of the CMSSM
parameter space that yield an
acceptable relic density and satisfy other phenomenological constraints
may be displayed in the  $(m_{1/2}, m_0)$ plane.
In Fig. \ref{fig:tb40},  the dark (blue)
shaded region corresponds to that portion of the CMSSM plane
with $\tan \beta = 40$, $A_0 = 2.5 m_0$, and $\mu > 0$ such that the computed
relic density yields the WMAP value given in Eq. (\ref{wmapden}).
For this choice of $\tan \beta$ and $A_0$, the relic density strip
is v-shaped. Inside the `v', the  annihilation cross sections
are too small to maintain an acceptable relic density and $\Omega_\chi h^2$ is too large.
The upper side of the `v', at large $m_0$, is produced by
co-annihilation processes between the LSP and the next lightest sparticle 
(in this case the $\tilde t$). These enhance the annihilation cross section and reduce the
relic density.  This occurs when the LSP and NLSP are nearly degenerate in mass.
The lower side of the `v', at lower $m_0$, is produced by coannihilations between the 
LSP and the $\tilde \tau$.
The dark (brown) shaded regions outside of the `v' have either $m_{\tilde t}< m_\chi$ 
or $m_{\tilde \tau}< m_\chi$
and are excluded.   Also shown in the figure is the constraint from $b \to s \gamma$ \cite{bsgex}
(shaded green) which excludes the stop-coannihilation strip.  Contours of constant Higgs mass
are shown by the red dot-dashed curves. Higgs masses are computed using FeynHiggs \cite{fh} 
and carry a roughly 1.5 GeV uncertainty. The thick purple line corresponds to the 
ATLAS limit on supersymmetry searches \cite{lhc}.  The area to left of the line is excluded.
Finally, the sold green contours correspond to the ratio of the branching fraction
of $B_s \to \mu^+ \mu^-$ relative to the Standard Model. A ratio of 1.5 corresponds to 
the 95 \% CL upper limit from the recent result from LHCb \cite{:2012ct}
and 1.3 to the 95 \% CL upper limit when all experiments are combined.
 

\begin{figure}
  \includegraphics[width=.5\textwidth]{Astro/Figures/m0vM8A2.5m0_40ses.eps}
   \caption{\it The $(m_{1/2}, m_0)$ plane for $\tan \beta = 40$ and
   $\mu > 0$, assuming $A_0 = 2.5 m_0, m_t = 173.2$~GeV and
   $m_b(m_b)^{\overline {MS}}_{SM} = 4.25$~GeV. Contours and shaded
   regions are described in the text.}  \label{fig:tb40}
\end{figure}

Note that the choice $A \ne 0$ is made to ensure a sufficiently large Higgs mass.
For $A_0 = 0$, the maximum Higgs mass along the stau-coannihilation strip is
only slight greater than 120 GeV, far short of the value reported in the recent
LHC results \cite{lhch}. Therefore, only the upper end of the strip is compatible with
a Higgs mass around 125 -- 126 GeV and a branching fraction for $B_s \to \mu^+ \mu^-$
sufficiently close to the Standard Model value.



\paragraph{NUHM}

One possible generalization of the CMSSM is the so-called NUHM
in which the Higgs soft masses are not constrained to be equal to 
$m_0$. Indeed, as the Higgses are typically found in separate multiplets in 
a grand unified theory, one or both of the Higgs soft masses may be independent.
In the NUHM1, we may set $m_1 = m_2 \ne m_0$, where $m_{1,2}$ are the 
soft masses associated with $H_{1,2}$. Instead of $m_{1,2}$, one may choose
{\em either} $\mu$ {\em or} the Higgs pseudo-scalar mass, $m_A$ (which is 
a surrogate for $B$) as a free parameter in addition to $m_0$.
In the NUHM2, both $m_1$ and $m_2$ are free and one can equivalently
choose {\em both} $\mu$ {\em and} $m_A$ as free parameters. 

In Fig. \ref{fig:muma}, we show one example of a $\mu, m_A$ plane
with $\tan \beta = 30$, $m_{1/2} = m_0 1000$ GeV,
and $A_0 = 2.5 m_0$. The strips of acceptable relic density now form a cross-like 
shape. Outside the cross, the relic density is too large. 
The horizontal part of the crosses are due to an enhanced cross section through
rapid s-channel annihilation through the heavy Higgses. For $m_{1/2} = 1000$ GeV,
the neutralino mass, is roughly 430 GeV and the funnel-like region occurs
when $m_A \approx 2 m_\chi$. In contrast, the vertical part of the cross occurs
when $\mu$ becomes sufficiently small that the the LSP picks up a 
significant Higgsino component (at large $|\mu|$, it is almost pure bino) 
which enhances certain final state annihilation channels such as $W^+ W^-$.  


\begin{figure}
  \includegraphics[width=.5\textwidth]{Astro/Figures/mumAs_30_2.5_1000_1000s.eps}
   \caption{\it The $(\mu, m_A)$ plane for  $\tan \beta = 30$, $m_{1/2} = m_0 = 1000$ GeV,
assuming $A_0 = 2.5 m_0, m_t = 173.2$~GeV and
$m_b(m_b)^{\overline {MS}}_{SM} = 4.25$~GeV. Contours and shaded regions are
described in the text. }
  \label{fig:muma}
\end{figure}

Most of the region in Fig. \ref{fig:muma} with $\mu < 0$ is excluded by $b \to s \gamma$
and for $\mu > 0$, the region with $m_A \agt 1000$ GeV has a sufficiently small 
branching fraction for $B_s \to \mu^+ \mu^-$. On the other hand, the Higgs mass is 
$\agt 124$ GeV across the plane and $\agt 125$ GeV for most of the area with $\mu > 0$.
The vertical dashed black lines at small $|\mu|$ correspond to a chargino mass
at the lower limit of 104 GeV.



\paragraph{The pMSSM}


\paragraph{NMSSM}
The Next-to-Minimal Supersymmetric Standard Model
(NMSSM) is a simple extension of the MSSM that contains
an additional gauge singlet superfield. The vev of this singlet
induces an effective $\mu$ term that is naturally of the order
of the electroweak scale, thus providing a solution to
the naturalness problem~\cite{Ellwanger:2009dp}. The model contains one additional
neutralino state, the singlino, as well as three scalar
($h_1,h_2,h_3$) and two pseudoscalar ($a_1,a_2$) Higgs bosons.
 An
important feature of the model is that the singlet fields can
be very light and escape the LEP bounds. This is because
these fields mostly decouple from the SM fields. 
 Furthermore a large mixing with the singlet can modify the properties of the SM-like Higgs, allowing quite naturally for $m_h=126$~GeV as well as an enhanced rate for its decay into two-photons.
As concerned dark matter, the NMSSM shares many of the characteristics of the MSSM. The main differences occur a)  when the LSP has some singlino component b) when the Higgs sector contains new light states that play a role in dark matter interactions. For example new Higgs states can enhance greatly DM annihilation when $m_\chi\approx m_{h,a}/2$ or can provide  new annihilation channels when they can be produced in the final state. As a consequence the NMSSM allows for the possibility of light neutralinos (much below $M_Z/2$), 
that annihilate efficiently through the exchange of light
Higgs singlets or  into light Higgs singlets ~\cite{Vasquez:2010ru}. The model also accommodates the possibility of a gamma-ray line at 130 GeV, without violating any other constraints from cosmic rays. This requires fine-tuning of the parameters such that 1) the mass of a pseudoscalar is precisely twice the neutralino mass  and 2) the annihilation of the pseudoscalar is dominantly into two-photons rather than into quarks ~\cite{Das:2012ys}.

\subsubsection{Universal Extra Dimensions}

Extra dimension models also propose a WIMP dark matter candidate. The UED scenario [1] where all standard model particles are allowed to propagate freely in the bulk is of particular interest. In this model momentum conservation in the
extra dimensions entails conservation of  a KK number. Orbifolding is required to obtain
chiral zero modes from bulk fermions, and breaks extra dimensional momentum conservation. However, there remains a discrete subgroup, KK parity, thus the lightest KK-odd
particle is stable. In the minimal universal extra dimension model (MUED) the dark mat-
ter candidate is in general a vector particle, $B_1$, the Kaluza-Klein (KK) level 1 partner
of the U(1) gauge boson. 
In the MUED model all KK states of a given level have nearly the same mass at tree-
level, n/R, where R is the size of the compact dimension. The mass degeneracy is lifted
only by standard model (SM) masses and by  radiative corrections. These mass splittings are however small
for all weakly interacting particles. This means that co-annihilation channels naturally
play an important role in the computation of the relic abundance of dark matter. 
Furthermore since the level 2 particles are close to twice the mass of those of level 1, annihilation or co-annihilation processes can easily be enhanced by resonance effect. When including level 2 particles in the computation, the preferred scale for DM was found to be  around 1.35 TeV~\cite{Belanger:2010yx}. 
Going beyond the MUED framework one can treat mass splittings as free parameters, shifting significantly the preferred 
DM mass, for example in the limit where the coannihilation processes are negligible the DM mass is around 800GeV.
The measurement of the Higgs mass and of its couplings at the LHC can be used to put a lower limit on the scale $R$. Indeed light KK particles, in particular the KK top,   lead  to an increase in the $hgg$ coupling and to a  decrease in the $h\gamma\gamma$ coupling, and to a lower bound on $R>500$~GeV~\cite{Belanger:2012mc}. 
One characteristics of MUED DM is that annihilation in the galaxy has a large fraction into fermions leading to strong signal into positrons, however the large mass scale makes  the signature unlikely to be observable.
 



\subsubsection{Higgs Portal Models}

\paragraph{The Model}

The simplest extension of the SM is the addition of a real singlet scalar field.Although it is possible to generalize to scenarios with more than one singlet, the simplest
case of a single additional singlet scalar provides a useful framework to analyze
the generic implications of an augmented scalar sector to the SM.
The most general renormalizable potential involving the SM Higgs doublet $H$ and the
singlet $S$ is
\bea
{\cal L}&=& {\cal L}_{SM} + (D_{\mu}H)^\dag (D^{\mu}H) + \frac{1}{2} \mu_H^2 H^\dag H 
-\frac{1}{4}\lambda_H H^4
\nonumber
\\
&+& \frac{1}{2} \partial_{\mu}S \partial^{\mu}S
-\frac{\lambda_{S}}{4} S^4 - \frac{\mu_S^2}{2} S^2 - \frac{\lambda_{HS}}{4}S^2 H^{\dag}H
\nonumber
\\
&-&\frac{\kappa_1}{2} H^\dag H S - \frac{\kappa_3}{3}S^3 - V_0
\label{Eq:Lagrangian}
\eea 
  where $D_{\mu}$ represents the covariant derivative.
 We have eliminated a possible linear term in $S$ by a constant shift,
absorbing the resulting S-independent term in the vacuum energy $V_0$. 
We require that the minimum of the potential occur at $v =$ 246 GeV . Fluctuations
around this vacuum expectation value are the SM Higgs boson.
 For the case of interest here for which $S$ is stable and may be a dark matter candidate,
we impose a $Z_2$ symmetry on the model, thereby eliminating the $\kappa_1$ and $\kappa_3$  terms. 
 We also require that the true vacuum of the theory satisfies $\langle S \rangle=0$, thereby precluding
  mixing of $S$ and the SM Higgs boson and the existence of cosmologically problematic domain walls.
More generally, one can also have a dim-4   vector Higgs portal, which couples
the Higgs doublet to a massive    
vector field $X_\mu$ from the hidden sector,
\begin{eqnarray}
\Delta {\cal L}_{\rm vector} &=& {\lambda_{hv} \over 4} ~ \bar H H~ X_\mu X^\mu + ( \xi_1 ~
\bar H iD_\mu H ~ X^\mu  \nonumber\\
&+& \xi_2 ~ \bar H H~ i \partial_\mu X^\mu +
{\rm h.c.}) \;, 
\label{vector-portal}
\end{eqnarray}
where the covariant derivative $D_\mu$  is taken with respect to the Standard Model (SM) gauge
group.\footnote{For generality, we have included the $\partial_\mu X^\mu$ term,
which may be relevant in models with field--dependent mass terms. }
 $X_\mu$ can be associated with a hidden U(1). It  becomes massive
due to the Higgs or St\"uckelberg mechanism in the hidden sector. 



Following the model independent approach of Ref.~\cite{Kanemura:2010sh}, we can 
also consider  a third possibility : dark matter  can consist of Majorana fermions $\chi$   which interact with  the SM fields
only through the Higgs-portal. The stability of the DM particle is ensured by a $Z_2$
parity, whose origin is  model--dependent. For example, in the  vector case it
stems  from a natural parity symmetry of abelian gauge sectors with minimal
field content \cite{Lebedev:2011iq}.   The relevant  terms in the 
Lagrangians  are 
\begin{eqnarray} \!&&\Delta {\cal L}_S = -{1\over 2} m_S^2 S^2 - {1\over 4}
\lambda_S S^4 -  {1\over 4} \lambda_{hSS}  H^\dagger H  S^2 \;, \nonumber \\
\!&&\Delta {\cal L}_V = {1\over 2} m_V^2 V_\mu V^\mu\! +\! {1\over 4} \lambda_{V} 
(V_\mu V^\mu)^2\! +\! {1\over 4} \lambda_{hVV}  H^\dagger H V_\mu V^\mu ,
\nonumber \\ \! &&\Delta {\cal L}_f = - {1\over 2} m_f \bar \chi \chi -  {1\over 4}
{\lambda_{hff}\over \Lambda} H^\dagger H \bar \chi \chi \;.   \end{eqnarray}




Related ideas and analyses can be found in  \cite{Lebedev:2011iq,all1,Peter,Andreas:2010dz,all2} and more  recent studies of Higgs-portal scenarios have appeared in
\cite{all3,Chu:2011be}. 


The properties of the dark matter particles can be studied in direct detection
experiments.  The DM interacts elastically with nuclei through the Higgs boson
exchange. The  resulting nuclear recoil is then interpreted in terms of the DM
mass and  DM--nucleon cross section.  The spin--independent DM--nucleon
interaction can be found in  \cite{Kanemura:2010sh}
Moreover, if the DM particles are light enough, $M_{\rm DM} \leq \frac12 m_h$, they will
appear as  invisible decay products of the Higgs boson. For the various cases, 
the Higgs partial decay  widths into invisible DM particles are given by
\begin{eqnarray}
 &&\Gamma^{{\rm inv}}_{h\rightarrow SS} = \frac{\lambda_{hSS}^2 v^2 \beta_S}{64 \pi  m_h}  \;, \nonumber\\
&& \Gamma^{\rm inv}_{h \rightarrow V V} = \frac{\lambda^2_{hVV} v^2 m_h^3
\beta_V }{256 \pi   M_{V}^4}
\left( 1-4 \frac{M_V^2}{m_h^2}+12\frac{M_V^4}{m_h^4}
\right), \nonumber\\
&&  \Gamma^{\rm inv}_{h \rightarrow \chi \chi} = {\lambda_{hff}^2 v^2 m_h 
\beta_f^{3}\over 32 \pi 
\Lambda^2 }  \;, 
\end{eqnarray}
where $\beta_X=\sqrt{1-4M_X^2/m_h^2}$. 


\paragraph{Astrophysical  consequences}


Then, we can  derive constraints on the various DM particles
from the  WMAP satellite \cite{wmap} and from the current direct detection 
experiment XENON100 \cite{Aprile:2012nq}, and to make predictions  for future
upgrades of the latter experiment, assuming that  the  Higgs boson  has a mass
$m_h =125$ GeV and is approximately SM--like such  that its invisible decay 
branching ratio is smaller than 10\%; we have checked that increasing this
fraction  to 20\%  does not change our results significantly.





We find that light dark matter,  $M_{\rm DM} \alst 60 $ GeV, violates the bound
on the invisible Higgs decay branching ratio and thus is excluded. This applies
in particular to the case of  scalar DM with a mass of 5--10 GeV considered, 
for instance, in  Ref.~\cite{Andreas:2010dz}. On the other hand, heavier dark
matter, particularly for $M_{\rm DM} \agt 80 $ GeV,  is allowed  by both  
${\rm BR}^{\rm inv}$ and XENON100.  We note that almost the entire available
parameter space will be probed by the XENON100 upgrade. The exception is a small
resonant region around 62 GeV, where the Higgs--DM coupling is extremely  small.




\begin{figure}
    \includegraphics[width=.5\textwidth]{Astro/Figures/Sigma2012}
          \caption{
Spin independent DM--nucleon cross section 
versus DM mass.
The upper band (3)  corresponds to fermion DM, the middle one (2)
to vector DM and the lower one (1)   to scalar DM. The solid, 
dashed and dotted lines represent XENON100 (2012 data \cite{Aprile:2012nq}), XENON100 upgrade
and XENON1T sensitivities, respectively.
 }
\label{Fig:SigmaSIbis}
\end{figure}



This can be seen from  Fig.~\ref{Fig:SigmaSIbis}, which displays
predictions for the spin--independent  DM--nucleon cross section  $\sigma_{\rm
SI}$ (based on the lattice $f_N$)    subject to the WMAP and  ${\rm BR}^{\rm
inv} < 10\%$ bounds. 
The prospects
for the upgrade of XENON100 (with a projected sensitivity corresponding to  
60,000 kg-d, 5-30 keV and 45\% efficiency)   and XENON1T are shown   by the
dotted lines. 
We find that light dark matter,  $M_{\rm DM} \alst 60 $ GeV, violates the bound
on the invisible Higgs decay branching ratio and thus is excluded. This applies
in particular to the case of  scalar DM with a mass of 5--10 GeV considered, 
for instance, in  Ref.~\cite{Andreas:2010dz}
The upper band  corresponds to the fermion Higgs-portal DM
and is excluded by XENON100. On the other hand, scalar and vector DM are both
allowed for a wide range of masses. Apart from a very small region around
$\frac12 m_h$, this parameter space will be probed by  XENON100--upgrade and XENON1T. The
typical value for the scalar  $\sigma_{\rm SI }$ is a few times $10^{-9}$ pb,
whereas $\sigma_{\rm SI }$ for vectors is larger by a factor  of 3 which
accounts for the number of  degrees of freedom.



\subsubsection{Other Models}

\subsection{Dark Matter at the LHC}
Direct searches for supersymmetry at  the LHC have had a significant impact on the allowable
regions of the supersymmetric parameter space particularly in the 
context of the CMSSM. An example of this is shown by the
purple curve in Fig. \ref{fig:tb40}. For relatively low $m_0$,
the most recent results from ATLAS place a lower bound on 
$m_{1/2}$ of roughly 700 GeV.  Perhaps of greater significance is the discovery of
the candidate Higgs at 125-126 GeV. While consistent with 
general predictions in supersymmetric models that $m_h \alst 128 - 130$ GeV,
a 125 GeV Higgs lies at the edge of what can be obtained and pushes
the model to require large contributions from stop mixing (hence a large value of 
$A_0$ in the CMSSM) and relatively large SUSY masses. Of course
large SUSY masses are consistent with the lack of discovery of supersymmetric
particles at the LHC, and are consistent with little or no departures
from the standard model in rare B decays. Of course this can not be viewed as a 
ringing endorsement for supersymmetry. Indeed the past prospect of resolving
the discrepancy between theory and experiment for the anomalous magnetic moment
of the muon, has now essentially evaporated.   

To account for the recent LHC results along with other low energy observables,
it is better to perform a global likelihood analysis which can identify regions of the 
parameter space which best fit the data. 
It is well established that Markov-Chain Monte-Carlo (MCMC) algorithms 
offer an efficient technique for sampling a large parameter space such as 
the CMSSM or its variants.  MCMC has been utilized in the Mastercode \cite{mcweb}
framework to perform a frequentist analysis of the CMSSM and other variants of the model.
The MCMC technique is used to sample the SUSY parameter space,
and thereby construct the $\chi^2$ probability function,
$P(\chi^2,N_{\rm dof})$. This accounts for the number of degrees of
freedom, $N_{\rm dof}$, and thus provides a quantitative measure for the
quality-of-fit such that $P(\chi^2,N_{\rm dof})$ can be used to estimate the
absolute probability with which the CMSSM describes the experimental data. 

The results of the mastercode analysis include the parameters of the
best-fit points as well as the 68 and
95\%~C.L.\ regions  
found with default implementations of the phenomenological, experimental
and cosmological constraints. These include precision electroweak data,
the anomalous magnetic moment of the muon,  
$B$-physics observables, the Higgs
  boson mass, $m_h$, and the cold dark matter (CDM) density.
In addition it includes
the constraint imposed by the experimental
upper limit on the spin-independent DM scattering
cross section from XENON100 \cite{Aprile:2012nq}. 
The results described here are taken from \cite{Buchmueller:2008qe,Buchmueller:2011sw,Buchmueller:2012hv}.

In Fig. \ref{fig:mc}, we show the resulting 68 \% (shown in red)
and 95 \% (shown in blue) CL limits from the mastercode analysis \cite{Buchmueller:2012hv} 
in the $m_0,m_{1/2}$
plane corresponding to $\Delta \chi^2 = 2.3$ and 5.99
relative to the best fit point  (note the axes are reversed compared to Fig. \ref{fig:tb40}).
Results which include the ATLAS constraints at 5/fb are shown by solid curves. The best
fit point is at ($m_0, m_{1/2}$) = (300,910) GeV and is shown by the filled star. 
At the best fit point, we also have $A_0 \simeq 1300$ GeV, and $\tan \beta = 16$
We see in Fig.~\ref{fig:mc} that the 95\% CL region in the CMSSM extends 
to $m_0 \sim 4000$ GeV and $m_{1/2} \sim 2400$ GeV. 
Note that the CMSSM fit features two
disconnected 68\%~CL `islands', the one at lower $m_0$ and $m_{1/2}$
corresponding to the stau coannihilation region, and that at larger $m_0$
and $m_{1/2}$ corresponding to the s -channel rapid-annihilation funnel region
(the best fit point in the upper island has $\tan \beta = 46$. 
However, the MC sampling also includes a few intermediate points
that also have $\Delta \chi^2 < 2.30$, reflecting the relative flatness of
the global $\chi^2$ function along the band between $(m_0, m_{1/2}) \sim
(300, 900)$ GeV and $\sim (1100, 1900) $ GeV. Typically, these points
sit in rapid-annihilation funnels, and it is possible that a more
complete sampling might reveal a lower `isthmus'  connecting these
islands.


\begin{figure}
  \includegraphics[width=.5\textwidth]{Astro/Figures/mc78cmssms}
   \caption{\it The $(m_0, m_{1/2})$ planes in the CMSSM including the ATLAS 5/fb
   constraint  assuming $m_h = 125 \pm 1 ~({\rm exp.}) \pm 1.5 ~({\rm theo.})$
GeV. The most recent results are indicated by solid lines
  and filled stars, and previous fit based on $\sim 1$/fb of LHC data
  is indicated by dashed lines and open stars.    The blue lines denote
  68\%~CL  contours, and the red lines denote 95\%~CL contours.
  The dotted lines correspond to the pre-LHC predictions based on the
  available low energy data.}
  \label{fig:mc}
\end{figure}

The impact of the recent LHC results can be seen by comparing the solid curves to the
the dashed and dotted curves in Fig. \ref{fig:mc}. The dotted curves correspond to 
the pre-LHC expectations \cite{Buchmueller:2008qe,Buchmueller:2011sw} and were
driven by a large extent by $g_\mu -2$. The initial best fit result 
was found at quite low susy masses with $(m_0, m_{1/2}) \sim
(90, 360)$ GeV and had a p-value of 37\%. It position is shown by an 
open star. As one can see the entire pre-LHC 68\% CL region is now
excluded at 95\% CL, though much of the initial 95\% CL region is still valid and includes
the current best fit.  The dashed curves in Fig. \ref{fig:mc} represent the status of 
the CMSSM after 1/fb data were collected though assuming a 125 GeV Higgs boson mass.
The best fit point in this case is at large $m_0, m_{1/2}$ also shown by an open star. 
The p-value in this case is only 12\% and increases only to 15\% if one drops the Higgs
mass constraint. Thus already at 1/fb, the LHC results had greatly diminished
the probability that the CMSSM improves the fit relative to the Standard Model.
The current results have a p-value of 8.5\% which is close to the Standard Model
value.  Of course the Standard Model p-value does not include the dark matter
constraint as there is no candidate for dark matter within the Standard Model.



\subsection{Other searches}

\subsubsection{Direct Detection}

Direct searches of DM particles through 
their scattering off  nuclei in a large detector can establish that the DM matter is indeed made of a new stable particle. 
The elastic scattering of weakly interacting massive particles (WIMPs) off nuclei 
taking place at low momentum transfer, it can be conveniently describe in term of an effective Lagrangian describing the interaction of DM with quarks and gluons giving rise to either spin independent or spin dependent interactions.
The spin independent(SI) cross section for WIMPs on nuclei adds coherently and is proportional to the square of the number of nucleons, it therefore usually dominates for heavy nuclei. 
The spin independent cross section receives a contribution from Higgs exchange, Z exchange (except for Majorana fermions)
and from interactions with new colored fermions/scalars (for example new quarks in extra dimension models or squarks in supersymmetry). The latter contribution is however constrained by the non-observation of new colored particles at the LHC. The spin dependent (SD) cross section depend solely on the nucleon that contributes to the nucleus spin, and is dominant only for light nuclei. 
The SD cross section receives contribution from Z exchange and/or from interactions with new colored fermions/scalars.
In order to easily compare results obtained using different nuclei,
limits are normally expressed in terms of the SI or SD interaction with protons and neutrons. 
 At the microscopic level a positive signal in several DM direct searches could altogether lead to information on up to four independent quantities that depend on the details of the DM model, the SD/SI interactions on protons and neutrons. Note however that when scalar interactions are dominated by Higgs exchange the cross-section on protons and neutrons are almost equal.
 Furthermore, if the DM has a mass comparable or below that of the nucleus, the shape of the nucleus recoil energy distribution can also be used to extract some rough information of the DM mass.
 
 \begin{figure}[tb]
\begin{center}
  \includegraphics[width=.4\textwidth]{Astro/Figures/SI_result}
\caption{Limits on spin-independent direct detection cross section $\sigma_{\text{SI}}$  on protons \textit{vs.}  dark matter mass $m_{DM}$. In grey
the preferred region in the CMSSM, from a combination of~\cite{Strege:2011pk,Fowlie:2012im,Buchmueller:2011ab}. }
\label{fig:si}
\end{center}
\end{figure}

Several experiments have been taking data, some claiming potential signals compatible with the 
detection of a weakly interacting massive particle. This includes DAMA~\cite{Bernabei:2010mq} which observes an annual modulation,  CoGeNT~\cite{Aalseth:2011wp} and CRESST~\cite{Angloher:2011uu} which also have found signals that would be compatible with dark matter in the range 5-30 GeV. These observations are however in conflict with the negative search results by other collaborations notably
CDMS, Edelweiss~\cite{Armengaud:2012kd} or XENON~\cite{Aprile:2012nq}. 
The large ton scale detectors that are planned (XENON, DEAP,DARWIN) should improve by more than one order of magnitude the current sensitivity  thus resolving the apparent conflict in SI results at low masses and probing a large number of DM models, see fig.~\ref{fig:si} for a comparison of current limits with expectations in the CMSSM. In particular, the case where the neutralino is a mixed gaugino/higgsino state  is challenged by current limits as illustrated in fig.~\ref{fig:higgsino} where $P=min(f_h,1-f_h)$ and $f_h$ is the higgsino fraction. 
Finally COUPP~\cite{Behnke:2008zza}, KIMS, Picasso~\cite{Archambault:2009sm} (Xenon10~\cite{Angle:2008we}) have set limits on  spin dependent interactions on protons (neutrons).



\begin{figure}[tb]
\begin{center}
  \includegraphics[width=.4\textwidth]{Astro/Figures/HfractionMLSPnat}
\caption{Spin-independent direct detection cross section
  $\sigma_{\text{SI}}$ on protons \textit{vs.}  dark matter mass
  $m_{LSP}$. The black (blue) line are the 90\% CL
  limits from the XENON100(2011) \cite{Aprile:2011hi} and (2012)
  results \cite{Aprile:2012nq}. The dashed brown line is the projected
  sensitivity of the XENON1T experiment \cite{Aprile:2012zx}. The
  color code shows the with $P>0.2$ (red), $0.1<P<0.2$ (orange)
  $0.01<P<0.1$ (green) and $0.001<P<0.01$ (blue). Note however that
  the relic density constraint is not imposed here.}
\label{fig:higgsino}
\end{center}
\end{figure}




\subsubsection{Indirect Detection}

In general, the goal of the ongoing generation of indirect experiments sensitive to dark matter is:
\begin{itemize}
\item[I.] to probe the vanilla ``WIMP paradigm'', at least for particles
of masses of the $\simeq {\cal O}(100)\,$GeV scale and characterized by S-wave annihlation cross section $\langle \sigma v\rangle$.

\item[II.] to clarify some of the ``anomalies'' presently claimed.

\item[III.] in case of independent detection (at colliders or direct detection), provide a cross-check or actually several ones, using the multi-messenger
characteristics of this detection strategy.
\end{itemize}

Concerning the first task, it is worth pointing out that for some channels the Fermi-LAT has already reached the sensitivity to test this paradigm  up to a few tens
of GeV (dwarf spheroidals~\cite{Ackermann:2011wa,GeringerSameth:2011iw}, diffuse gamma-ray halo signal~\cite{Ackermann:2012rg}) or even more for the Galactic Center~\cite{Hooper:2012sr}.

In general, we expect that probing the $\sim$100 GeV mass scale will be within reach with a decade worth of data, see for example the forecasts in~\cite{Baltz:2008wd}.
Especially for candidates annihilating into leptons, such a goal seems also within reach of Planck, which probes dark matter energy deposition at early
stage via its impact on the reionization (see e.g.~\cite{Galli:2009zc})



Needless to say, if new states are below the TeV scale, such kind of WIMP candidates are also in the right ball-park to be probed directly or indirectly by a future ILC,
hence the complementarity of the two.

The current generation of ground-based imaging atmospheric cherenkov telescopes (IACTs) is  less sensitive to theoretically preferred values of $\langle \sigma v\rangle$. 
Nonetheless, they are already more sensitive than Fermi-LAT to TeV scale dark matter,  see e.g.~\cite{Abramowski:2011hc}, and with the future CTA they may probe
not-yet-excluded regions of parameter space for viable particle physics model, see e.g.~\cite{Bergstrom:2010gh}.  Typically, the Galactic Center is among the most
promising targets, provided that the dark matter distribution is comparable to what expected based on pure cold dark matter simulation or even enhanced as a consequence
of baryons. {\it of course, playing with ``boost factors'' anything goes \ldots}



Performances similar to Fermi-LAT (but more dependent on astrophysical modeling of cosmic ray transport) are expected by high-precision measurements of cosmic ray
antimatter, most notably antiprotons and, possibly, anti-deuterons. Positrons are significantly sensitive to astrophysical backgrounds (see e.g.~\cite{Serpico:2011wg}) and both their primary and secondary fluxes show a larger dependence from source distribution (in space and time) as well as from  the medium properties (e.g. their E-losses crucially depend on B-field and interstellar
radiation fields). While they remain challenging for a {\it robust  detection} of dark matter, they may be useful for cross-checks of tentative signals.
AMS-02 and, concerning anti-deuterons, GAPS, are expected to achieve the needed precision and sensitivity for such competitive results. {\it here is the problem of lack of proper references substantiating the above point; this is done in several specific papers, though, such as 0909.2799 \ldots}

A caveat is mandatory: ultimately, if sufficient statistics is accumulated, the main limitations will come from the degree of understanding of the astrophysical foregrounds, so that
most of these projections must be taken with a grain of salt. 

An example of the second type of goal has been provided in the recent past by the multi-messenger constraints on the dark matter interpretation of the PAMELA positron fraction
``rise'' (where the relevance of the point just made clearly manifested) or, at present, by the tentative hint for a $\sim 130\,$GeV ``gamma-ray line''~\cite{Weniger:2012tx}.  For this kind of task, statistics helps a lot but it is clearly not enough. Cross-checks and tests with different techniques and possibly improved resolutions are needed.
Fortunately, current (HESS) or planned  (CTA) IACTs may provide such a tool. This is also an arena where the proposed satellite experiment Gamma-400~\cite{Galper:2012fp} might contribute, thanks to its superior resolution (see e.g.~\cite{Bergstrom:2012vd}).


The third possibility has been heavily discussed in recent years in the context of direct dection ``anomalies''  [\ldots]. If interpreted in terms of ``light'' dark matter,
a wealth of indirect detection cross-checks can be thought of, see e.g.~\cite{Hooper:2012ft,Hooper:2012gq}.
We conclude by pointing out that  especially in this context (cross-checking direct detection potential signals), neutrino signals from the center of the Sun
(and possibly the Earth) are of particular relevance. In fact, they probe a similar combination (albeit not equal!) of DM-baryon cross-section and local density of dark matter as direct detection
experiments.  
Significant advances are expected by the IceCube in its current configuration, including the Deep-core (see e.g.~\cite{Silverwood:2012tp}).
Further progress may be also possible if the R\&D PINGU low-energy extension will be realized~\cite{Koskinen:2011zz} (the same would apply to
comparable programs in the Mediterranean sea such as those pursed within Km3Net, of course). Finally, it is worth pointing out that this
is also one of the few ways to potentially detect indirectly  p-wave annihilating WIMPs, since the equilibrium flux is only dependent on the DM
scattering cross section.



\subsection{Dark Matter at the LC}


% For one-column wide figures use
%
% For two-column wide figures use
%\begin{figure*}
% Use the relevant command to insert your figure file.
% For example, with the graphicx package use
%  \includegraphics[width=0.75\textwidth]{Astro/Figures/example}
% figure caption is below the figure
%\caption{Please write your figure caption here. If you refer in the text to it, please use  `Fig.' }
%\label{fig:astro2}       % Give a unique label
%\end{figure*}
%
% For tables use
%\begin{table}
%% table caption is above the table
%\caption{Please write your table caption here. If you refer in the text 
%to it, please use  `Table'. }
%\label{tab:astro1}       % Give a unique label
%% For LaTeX tables use
%\begin{tabular}{lll}
%\hline\noalign{\smallskip}
%first & second & third  \\
%\noalign{\smallskip}\hline\noalign{\smallskip}
%number & number & number \\
%number & number & number \\
%\noalign{\smallskip}\hline
%\end{tabular}
%\end{table}


%\begin{acknowledgements}
%If you'd like to thank anyone, place your comments here
%and remove the percent signs.
%\end{acknowledgements}

% BibTeX users please use one of
%\bibliographystyle{spbasic}      % basic style, author-year citations
%\bibliographystyle{spmpsci}      % mathematics and physical sciences
%\bibliographystyle{spphys}       % APS-like style for physics
%\bibliography{}   % name your BibTeX data base

% Non-BibTeX users please use
\begin{thebibliography}{}
%
% and use \bibitem to create references. Consult the Instructions
% for authors for reference list style.
%
\bibitem{rot}
S. M. Faber and J. J. Gallagher,  {\it Ann. Rev. Astron.
Astrophys.} {\bf 17} (1979) 135;
A. Bosma, {\it Ap. J.} {\bf 86} (1981) 1825; V. C. Rubin, W. K.
Ford and N. Thonnard, {\it Ap. J.} {\bf 238} (1980) 471;	V. C. Rubin, D.
Burstein, W. K. Ford and N. Thonnard, {\it Ap. J.} {\bf 289} (1985) 81;
T. S. Van Albada  and R. Sancisi, {\it Phil. Trans. R. Soc. Land.} {\bf
A320} (1986) 447;
M. Persic and P. Salucci, {\it Ap. J. Supp.} {\bf 99} (1995) 501;
M. Persic, P. Salucci, and F. Stel, {\it MNRAS} {\bf 281} (1996) 27P;
 P.~Salucci, A.~Lapi, C.~Tonini, G.~Gentile, I.~Yegorova and U.~Klein,
  %``The Universal Rotation Curve of Spiral Galaxies. 2. The Dark Matter Distribution out to the Virial Radius,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 378}, 41 (2007)
  [astro-ph/0703115 [ASTRO-PH]].
  %%CITATION = ASTRO-PH/0703115;%%
  
  \bibitem{xray}
  D. Fabricant and P. Gorenstein, {\it Ap. J.} 
{\bf 267} (1983) 535;
	G. C. Stewart, C. R. Canizares, A. C. Fabian and P. E. J.
 Nilsen, {\it Ap. J.} {\bf 278}
 (1984) 53;
  W. Forman, C. Jones, and W. Tucker, {\it Ap. J.} {\bf 293}
(1985) 102; A. C. Fabian, P. A. Thomas, S. M. Fall, and R. E. White III, {\it
MNRAS} {\bf 221} (1986) 1049; M. Loewenstein and R. E. White, {\it Ap. J.}
{\bf 518} (1999) 50; M. Loewenstein and R. F. Mushotzky, astro-ph/0208090;
 J. S. Mulchaey, D. S. Davis, R. F. Mushotzky, and D. Burstein,
{\it Ap. J.} {\bf 404} (1993) L9;
M. J. Henriksen and G. A. Mamon, {\it Ap. J.} {\bf 421} (1994) L63;
L. P. David, C. Jones, and W. Foreman, {\it Ap. J.} 
{\bf 445} (1995) 578.

\bibitem{lense} J. A. Tyson, F. Valdes, and R. A. Wenk,
 {\it Ap. J.} {\bf 349} (1990) L1;
 Y. Mellier, {\it Ann. Rev. Ast. Astr.} {\bf 37} (1999) 127;
 L. van Waerbeke, Y. Mellier, and M. Radovich, {\it A. A.}
{\bf 374} (2001) 757; . Mellier, {\it Sp. Sci. Rev.} {\bf 100} (2002) 73.

\bibitem{both}
 D.~Wittman, {\it et al.},
  % ``First Results On Shear-Selected Clusters From the Deep Lens Survey: Optical
  %Imaging, Spectroscopy, and X-ray Followup,''
  Astrophys.\ J.\  {\bf 643}, 128 (2006)
  [arXiv:astro-ph/0507606];
  %%CITATION = ASTRO-PH 0507606;%%
  D.~Clowe,{\it et al.},
  %``A direct empirical proof of the existence of dark matter,''
   Astrophys.\ J.\  {\bf 648} (2006) L109
[arXiv:astro-ph/0608407].
  %%CITATION = ASTRO-PH/0608407;%%
  
  \bibitem{bao}
  W.~J.~Percival, S.~Cole, D.~J.~Eisenstein, R.~C.~Nichol, J.~A.~Peacock, A.~C.~Pope and A.~S.~Szalay,
  %``Measuring the Baryon Acoustic Oscillation scale using the SDSS and 2dFGRS,''
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 381}, 1053 (2007)
  [arXiv:0705.3323 [astro-ph]].
  %%CITATION = ARXIV:0705.3323;%%
  
  \bibitem{bbn}
  J.~-M.~Yang, M.~S.~Turner, G.~Steigman, D.~N.~Schramm and K.~A.~Olive,
  %``Primordial Nucleosynthesis: A Critical Comparison of Theory and Observation,''
  Astrophys.\ J.\  {\bf 281}, 493 (1984).
  %%CITATION = ASJOA,281,493;%%
  
    \bibitem{wmap}
  E.~Komatsu {\it et al.}  [WMAP Collaboration],
  %``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations:
  %Cosmological Interpretation,''
  Astrophys.\ J.\ Suppl.\  {\bf 192} (2011) 18
  [arXiv:1001.4538 [astro-ph.CO]].
  %%CITATION = APJSA,192,18;%%
  
  \bibitem{Hegyi:1985yu} 
  D.~J.~Hegyi and K.~A.~Olive,
  %``A Case Against Baryons in Galactic Halos,''
  Astrophys.\ J.\  {\bf 303}, 56 (1986).
  %%CITATION = ASJOA,303,56;%%
  
  \bibitem{pac}B. Paczynski, {\it Ap. J.} {\bf 304} (1986) 1;
C. Alcock {\it et al.}, {\it Nature} {\bf 365} (1983) 621;
E. Aubourg {\it et al.} {\it Nature} {\bf 365}
(1983) 623;
C. Alcock {\it et al.}, {\it Ap. J .} {\bf 542} (2000) 281;
T. Lasserre, {\it et al.}, {\it A. A.} {\bf 355} (2000) 39L;
C. Afonso {\it et al.}, Astron.\ Astrophys.\  {\bf 400}, 951 (2003).

  \bibitem{Hannestad:2010yi} 
  S.~Hannestad, A.~Mirizzi, G.~G.~Raffelt and Y.~Y.~Y.~Wong,
  %``Neutrino and axion hot dark matter bounds after WMAP-7,''
  JCAP {\bf 1008}, 001 (2010)
  [arXiv:1004.0695 [astro-ph.CO]].
  %%CITATION = ARXIV:1004.0695;%%
  
  \bibitem{lhch}
G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 1 (2012)
  [arXiv:1207.7214 [hep-ex]];
  %%CITATION = ARXIV:1207.7214;%%
   S.~Chatrchyan {\it et al.}  [CMS Collaboration],
  %``Observation of a new boson at a mass of 125 GeV with the CMS experiment at the LHC,''
  Phys.\ Lett.\ B {\bf 716}, 30 (2012)
  [arXiv:1207.7235 [hep-ex]].
  %%CITATION = ARXIV:1207.7235;%%
  
    \bibitem{bsgex}
S.~Chen {\it et al.}  [CLEO Collaboration],
%``Branching fraction and photon energy spectrum for b $\to$ s gamma,''
Phys.\ Rev.\ Lett.\  {\bf 87} (2001) 251807
[arXiv:hep-ex/0108032];
%%CITATION = HEP-EX 0108032;%%
P.~Koppenburg {\it et al.}  [Belle Collaboration],
%``An inclusive measurement of the photon energy spectrum in b $\to$ s gamma
%decays,''
Phys.\ Rev.\ Lett.\  {\bf 93} (2004) 061803
[arXiv:hep-ex/0403004].
%%CITATION = HEP-EX 0403004;%%
B.~Aubert {\it et al.}  [BaBar Collaboration],
%``Determination of the branching fraction for inclusive decays B $\to$ X/s gamma,''
arXiv:hep-ex/0207076;
%%CITATION = HEP-EX 0207076;%%
E.~Barberio {\it et al.}  [Heavy Flavor Averaging Group (HFAG)],
  %``Averages of b-hadron properties at the end of 2005,''
  arXiv:hep-ex/0603003.
  %%CITATION = HEP-EX/0603003;%%
  
  \bibitem{fh}
 G.~Degrassi, S.~Heinemeyer, W.~Hollik, P.~Slavich and G.~Weiglein,
  Eur.\ Phys.\ J.\ C {\bf 28} (2003) 133
  [arXiv:hep-ph/0212020];
  %%CITATION = HEP-PH 0212020;%%
   S.~Heinemeyer, W.~Hollik and G.~Weiglein,
  Eur.\ Phys.\ J.\ C {\bf 9} (1999) 343
  [arXiv:hep-ph/9812472];
  %%CITATION = HEP-PH 9812472;%%
  S.~Heinemeyer, W.~Hollik and G.~Weiglein,
  Comput.\ Phys.\ Commun.\  {\bf 124} (2000) 76
  [arXiv:hep-ph/9812320];
  %%CITATION = CPHCB,124,76;%%
   M.~Frank {\it et al.}, 
  JHEP {\bf 0702} (2007) 047
  [arXiv:hep-ph/0611326];
  %%CITATION = JHEPA,0702,047;%%
  See {\tt http://www.feynhiggs.de}~.

  
     \bibitem{lhc}
ATLAS Collaboration, \\
{\tt https://cdsweb.cern.ch/record/1472710/} {\tt files/ATLAS-CONF-2012-109.pdf}.


\bibitem{:2012ct} 
  RAaij {\it et al.}  [LHCb Collaboration],
  %``First evidence for the decay Bs -> mu+ mu-,''
  arXiv:1211.2674 [Unknown].
  %%CITATION = ARXIV:1211.2674;%%
  
\bibitem{Ellwanger:2009dp} 
  U.~Ellwanger, C.~Hugonie and A.~M.~Teixeira,
  %``The Next-to-Minimal Supersymmetric Standard Model,''
  Phys.\ Rept.\  {\bf 496}, 1 (2010)
  [arXiv:0910.1785 [hep-ph]].

\bibitem{Vasquez:2010ru} 
  D.~A.~Vasquez, G.~Belanger, C.~Boehm, A.~Pukhov and J.~Silk,
  %``Can neutralinos in the MSSM and NMSSM scenarios still be light?,''
  Phys.\ Rev.\ D {\bf 82}, 115027 (2010)
  [arXiv:1009.4380 [hep-ph]].


\bibitem{Das:2012ys} 
  D.~Das, U.~Ellwanger and P.~Mitropoulos,
  %``A 130 GeV photon line from dark matter annihilation in the NMSSM,''
  JCAP {\bf 1208}, 003 (2012)
  [arXiv:1206.2639 [hep-ph]].


\bibitem{Belanger:2010yx} 
  G.~Belanger, M.~Kakizaki and A.~Pukhov,
  %``Dark matter in UED: The Role of the second KK level,''
  JCAP {\bf 1102}, 009 (2011)
  [arXiv:1012.2577 [hep-ph]].


\bibitem{Belanger:2012mc} 
  G.~Belanger, A.~Belyaev, M.~Brown, M.~Kakizaki and A.~Pukhov,
  %``Testing Minimal Universal Extra Dimensions Using Higgs Boson Searches at the LHC,''
  arXiv:1207.0798 [hep-ph].
  
  \bibitem{Kanemura:2010sh}
  S.~Kanemura, S.~Matsumoto, T.~Nabeshima, N.~Okada,
  %``Can WIMP Dark Matter overcome the Nightmare Scenario?,''
  Phys. Rev.  {\bf D82} (2010)  055026;
  A.~Djouadi, O.~Lebedev, Y.~Mambrini and J.~Quevillon,
  %``Implications of LHC searches for Higgs--portal dark matter,''
  Phys.\ Lett.\ B {\bf 709} (2012) 65
  [arXiv:1112.3299 [hep-ph]].
  %%CITATION = ARXIV:1112.3299;%%

  
\bibitem{Lebedev:2011iq}
  O.~Lebedev, H.~M.~Lee and Y.~Mambrini,
  %``Vector Higgs-portal dark matter and the invisible Higgs,''
  arXiv:1111.4482 [hep-ph].
  %%CITATION = ARXIV:1111.4482;%%


\bibitem{all1}
  J.~McDonald,
  %``Gauge singlet scalars as cold dark matter,''
  Phys.\ Rev.\  {\bf D50 } (1994)  3637-3649;
%\bibitem{Burgess:2000yq}
  C.~P.~Burgess, M.~Pospelov, T.~ter Veldhuis,
  %``The Minimal model of nonbaryonic dark matter: A Singlet scalar,''
  Nucl.\ Phys.\  {\bf B619 } (2001)  709-728;
 %\bibitem{Davoudiasl:2004be}
  H.~Davoudiasl, R.~Kitano, T.~Li, H.~Murayama,
  %``The New minimal standard model,''
  Phys.\ Lett.\  {\bf B609 } (2005)  117-123;
%\bibitem{Patt:2006fw}
  B.~Patt and F.~Wilczek,
  %``Higgs-field portal into hidden sectors,''
  [hep-ph/0605188];
%\bibitem{He:2008qm}
  X.~-G.~He, T.~Li, X.~-Q.~Li, J.~Tandean, H.~-C.~Tsai,
  %``Constraints on Scalar Dark Matter from Direct Experimental Searches,''
  Phys.\ Rev.\  {\bf D79 } (2009)  023521;
   X.~-G.~He, T.~Li, X.~-Q.~Li, J.~Tandean, H.~-C.~Tsai,
  %``The Simplest Dark-Matter Model, CDMS II Results, and Higgs Detection at LHC,''
  Phys.\ Lett.\  {\bf B688 } (2010)  332;
%\bibitem{Barger:2010mc}
  V.~Barger, Y.~Gao, M.~McCaskey, G.~Shaughnessy,
  %``Light Higgs Boson, Light Dark Matter and Gamma Rays,''
  Phys.\ Rev.\  {\bf D82 } (2010)  095011;
%\bibitem{Barger:2007im}
  V.~Barger, P.~Langacker, M.~McCaskey, M.~J.~Ramsey-Musolf, G.~Shaughnessy,
  %``LHC Phenomenology of an Extended Standard Model with a Real Scalar Singlet,''
  Phys.\ Rev.\  {\bf D77 } (2008)  035005;
%\cite{Clark:2009dc}
%\bibitem{Clark:2009dc}
  T.~E.~Clark, B.~Liu, S.~T.~Love, T.~ter Veldhuis,
  %``The Standard Model Higgs Boson-Inflaton and Dark Matter,''
  Phys.\ Rev.\  {\bf D80}, 075019 (2009);
R.~N.~Lerner, J.~McDonald,
  %``Gauge singlet scalar as inflaton and thermal relic dark matter,''
  Phys.\ Rev.\  {\bf D80}, 123507 (2009);
O.~Lebedev, H.~M.~Lee,
  %``Higgs Portal Inflation,''
    [arXiv:1105.2284 [hep-ph]];
%\cite{arXiv:1106.3097}
%\bibitem{Andreas:2008xy}
  S.~Andreas, T.~Hambye, M.~H.~G.~Tytgat,
  %``WIMP dark matter, Higgs exchange and DAMA,''
  JCAP {\bf 0810 } (2008)  034;
%  [arXiv:1003.2595 [hep-ph]].
%\bibitem{Goudelis:2009zz}
  A.~Goudelis, Y.~Mambrini, C.~Yaguna,
  %``Antimatter signals of singlet scalar dark matter,''
  JCAP {\bf 0912 } (2009)  008;
%  [arXiv:0909.2799 [hep-ph]];
   C.~E.~Yaguna,
  %``Gamma rays from the annihilation of singlet scalar dark matter,''
  JCAP {\bf 0903} (2009) 003;
%  [arXiv:0810.4267 [hep-ph]].
  %%CITATION = ARXIV:0810.4267;%%
%\bibitem{Cai:2011kb}
  Y.~Cai, X.~-G.~He, B.~Ren,
  %``Low Mass Dark Matter and Invisible Higgs Width In Darkon Models,''
  Phys.\ Rev.\  {\bf D83 } (2011)  083524;
%  [arXiv:1102.1522 [hep-ph]].
%\bibitem{Biswas:2011td}
  A.~Biswas, D.~Majumdar,
  %``The Real Gauge Singlet Scalar Extension of Standard Model: A Possible Candidate of Cold Dark Matter,''
    [arXiv:1102.3024 [hep-ph]];
%\bibitem{Farina:2011bh}
  M.~Farina, M.~Kadastik, D.~Pappadopulo, J.~Pata, M.~Raidal, A.~Strumia,
  %``Implications of XENON100 results for Dark Matter models and for the LHC,''
   [arXiv:1104.3572 [hep-ph]];
%\cite{Hambye:2008bq}
%\bibitem{Hambye:2008bq}
  T.~Hambye,
  %``Hidden vector dark matter,''
  JHEP {\bf 0901}, 028 (2009);
%  [arXiv:0811.0172 [hep-ph]];
  %%CITATION = JHEPA,0901,028;%%
T.~Hambye and M.~H.~G.~Tytgat,
  %``Confined hidden vector dark matter,''
  Phys.\ Lett.\  B {\bf 683}, 39 (2010);
%  [arXiv:0907.1007 [hep-ph]].
  %%CITATION = PHLTA,B683,39;%%
%\cite{Hisano:2010yh}
%\bibitem{Hisano:2010yh}
  J.~Hisano, K.~Ishiwata, N.~Nagata and M.~Yamanaka,
  %``Direct Detection of Vector Dark Matter,''
  Prog.\ Theor.\ Phys.\  {\bf 126}, 435 (2011).
%  [arXiv:1012.5455 [hep-ph]].
  %%CITATION = PTPKA,126,435;%%


\bibitem{Peter} 
  C.~Englert, T.~Plehn, D.~Zerwas and P.~M.~Zerwas,
  %``Exploring the Higgs portal,''
  Phys.\ Lett.\ B\ {\bf 703}, 298  (2011);
  %%CITATION = PHLTA,B703,298;%%
C. Englert, T. Plehn, M. Rauch, D. Zerwas and P.M. Zerwas,
  arXiv:1112.3007 [hep-ph].



\bibitem{Andreas:2010dz}
  S.~Andreas, C.~Arina, T.~Hambye, F.~-S.~Ling, M.~H.~G.~Tytgat,
  %``A light scalar WIMP through the Higgs portal and CoGeNT,''
  Phys.\ Rev.\  {\bf D82 } (2010)  043522.


\bibitem{all2} 
In the context of Higgs-portal mirror matter, see also 
 R.~Foot, H.~Lew and R.~R.~Volkas,
  %``A Model with fundamental improper space-time symmetries,''
  Phys.\ Lett.\ B\ {\bf 272}, 67  (1991) 
  %%CITATION = PHLTA,B272,67;%%
  and
   A.~Melfo, M.~Nemevsek, F.~Nesti, G.~Senjanovic and Y.~Zhang,
  %``Inert Doublet Dark Matter and Mirror/Extra Families after Xenon100,''
  Phys.\ Rev.\ D {\bf 84} (2011) 034009.
  %%CITATION = ARXIV:1105.4611;%%
\bibitem{all3}
  Y.~Mambrini,
  %``Higgs searches and singlet scalar dark matter: when XENON100 meets the LHC,''
    [arXiv:1108.0671 [hep-ph]];
M.~Raidal, A.~Strumia,
  %``Hints for a non-standard Higgs boson from the LHC,''
  Phys.\ Rev.\  {\bf D84 } (2011)  077701.
  [arXiv:1108.4903 [hep-ph]];
 X.~-G.~He, J.~Tandean,
  %``Hidden Higgs Boson at the LHC and Light Dark Matter Searches,''
  Phys.\ Rev.\  {\bf D84 } (2011)  075018.
  [arXiv:1109.1277 [hep-ph]];
   Y.~Mambrini,
  %``Invisible Higgs and Scalar Dark Matter,''
  arXiv:1112.0011 [hep-ph].
  %%CITATION = ARXIV:1112.0011;%%
\bibitem{Chu:2011be}
  X.~Chu, T.~Hambye and M.~H.~G.~Tytgat,
  %``The Four Basic Ways of Creating Dark Matter Through a Portal,''
  arXiv:1112.0493 [hep-ph];
  %%CITATION = ARXIV:1112.0493;%%
%\bibitem{Ghosh:2011qc}
  K.~Ghosh, B.~Mukhopadhyaya and U.~Sarkar,
  %``Signals of an invisibly decaying Higgs in a scalar dark matter scenario: a study for the Large Hadron Collider,''
  Phys.\ Rev.\ D {\bf 84} (2011) 015017;
%  [arXiv:1105.5837 [hep-ph]];
  %%CITATION = ARXIV:1105.5837;%%
%\bibitem{Darkon} 
   I.~Low, P.~Schwaller, G.~Shaughnessy, C.~E.~M.~Wagner,
  %``The dark side of the Higgs boson,''
   [arXiv:1110.4405 [hep-ph]];
     M.~Pospelov, A.~Ritz,
  %``Higgs decays to dark matter: beyond the minimal model,''
  [arXiv:1109.4872 [hep-ph]];
%\bibitem{Weihs:2011wp}
R.~Foot, A.~Kobakhidze, R.~R.~Volkas,
  %``ATLAS and CMS hints for a mirror Higgs boson,''
  [arXiv:1109.0919 [hep-ph]];
E.~Weihs, J.~Zurita,
  %``Dark Higgs Models at the 7 TeV LHC,''
  [arXiv:1110.5909 [hep-ph]];
P.~J.~Fox, R.~Harnik, J.~Kopp, Y.~Tsai,
  %``Missing Energy Signatures of Dark Matter at the LHC,''
  [arXiv:1109.4398 [hep-ph]].

\bibitem{Micromegas}
  G.~Belanger, F.~Boudjema, A.~Pukhov and A.~Semenov,
  arXiv:1005.4133 [hep-ph]; 
  Comput.\ Phys.\ Commun.\  {\bf 180}, 747 (2009);
  Comput.\ Phys.\ Commun.\  {\bf 177}, 894 (2007).
  
  \bibitem{Aprile:2012nq}
  E.~Aprile {\it et al.}  [XENON100 Collaboration],
  %``Dark Matter Results from 225 Live Days of XENON100 Data,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 181301
  [arXiv:1207.5988 [astro-ph.CO]].
  %%CITATION = ARXIV:1207.5988;%%

\bibitem{Djouadi:2012zc}
  A.~Djouadi, A.~Falkowski, Y.~Mambrini and J.~Quevillon,
  %``Direct Detection of Higgs-Portal Dark Matter at the LHC,''
  arXiv:1205.3169 [hep-ph].
  %%CITATION = ARXIV:1205.3169;%%

  
  \bibitem{mcweb}
For more information and updates, please see {\tt http://cern.ch/mastercode/}.

\bibitem{Strege:2011pk} 
  C.~Strege, G.~Bertone, D.~G.~Cerdeno, M.~Fornasa, R.~Ruiz de Austri and R.~Trotta,
  %``Updated global fits of the cMSSM including the latest LHC SUSY and Higgs searches and XENON100 data,''
  JCAP {\bf 1203}, 030 (2012)
  [arXiv:1112.4192 [hep-ph]].

\bibitem{Fowlie:2012im} 
  A.~Fowlie, M.~Kazana, K.~Kowalska, S.~Munir, L.~Roszkowski, E.~M.~Sessolo, S.~Trojanowski and Y.~-L.~S.~Tsai,
  %``The CMSSM Favoring New Territories: The Impact of New LHC Limits and a 125 GeV Higgs,''
  Phys.\ Rev.\ D {\bf 86}, 075010 (2012)
  [arXiv:1206.0264 [hep-ph]].

\bibitem{Buchmueller:2011ab} 
  O.~Buchmueller, R.~Cavanaugh, A.~De Roeck, M.~J.~Dolan, J.~R.~Ellis, H.~Flacher, S.~Heinemeyer and G.~Isidori {\it et al.},
  %``Higgs and Supersymmetry,''
  Eur.\ Phys.\ J.\ C {\bf 72}, 2020 (2012)
  [arXiv:1112.3564 [hep-ph]].

\bibitem{Bernabei:2010mq} 
  R.~Bernabei {\it et al.}  [DAMA and LIBRA Collaborations],
  %``New results from DAMA/LIBRA,''
  Eur.\ Phys.\ J.\ C {\bf 67}, 39 (2010)
  [arXiv:1002.1028 [astro-ph.GA]].

\bibitem{Aalseth:2011wp} 
  C.~E.~Aalseth, P.~S.~Barbeau, J.~Colaresi, J.~I.~Collar, J.~Diaz Leon, J.~E.~Fast, N.~Fields and T.~W.~Hossbach {\it et al.},
  %``Search for an Annual Modulation in a P-type Point Contact Germanium Dark Matter Detector,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 141301 (2011)
  [arXiv:1106.0650 [astro-ph.CO]].


\bibitem{Angloher:2011uu} 
  G.~Angloher, M.~Bauer, I.~Bavykina, A.~Bento, C.~Bucci, C.~Ciemniak, G.~Deuter and F.~von Feilitzsch {\it et al.},
  %``Results from 730 kg days of the CRESST-II Dark Matter Search,''
  Eur.\ Phys.\ J.\ C {\bf 72}, 1971 (2012)
  [arXiv:1109.0702 [astro-ph.CO]].


\bibitem{Armengaud:2012kd}
  E.~Armengaud {\it et al.}  [EDELWEISS Collaboration],
  %``A search for low-mass WIMPs with EDELWEISS-II heat-and-ionization detectors,''
  Phys.\ Rev.\ D {\bf 86}, 051701 (2012)
  [arXiv:1207.1815 [astro-ph.CO]].

\bibitem{Aprile:2012nq} 
  E.~Aprile {\it et al.}  [XENON100 Collaboration],
  %``Dark Matter Results from 225 Live Days of XENON100 Data,''
  Phys.\ Rev.\ Lett.\  {\bf 109}, 181301 (2012)
  [arXiv:1207.5988 [astro-ph.CO]].

\bibitem{Behnke:2008zza} 
  E.~Behnke {\it et al.}  [COUPP Collaboration],
  %``Improved Spin-Dependent WIMP Limits from a Bubble Chamber,''
  Science {\bf 319}, 933 (2008)
  [arXiv:0804.2886 [astro-ph]].
  %%CITATION = ARXIV:0804.2886;%%

\bibitem{Archambault:2009sm} 
  S.~Archambault, F.~Aubin, M.~Auger, E.~Behnke, B.~Beltran, K.~Clark, X.~Dai and A.~Davour {\it et al.},
  %``Dark Matter Spin-Dependent Limits for WIMP Interactions on F-19 by PICASSO,''
  Phys.\ Lett.\ B {\bf 682}, 185 (2009)
  [arXiv:0907.0307 [hep-ex]].


\bibitem{Angle:2008we} 
  J.~Angle, E.~Aprile, F.~Arneodo, L.~Baudis, A.~Bernstein, A.~Bolozdynya, L.~C.~C.~Coelho and C.~E.~Dahl {\it et al.},
  %``Limits on spin-dependent WIMP-nucleon cross-sections from the XENON10 experiment,''
  Phys.\ Rev.\ Lett.\  {\bf 101}, 091301 (2008)
  [arXiv:0805.2939 [astro-ph]].

\bibitem{Aprile:2011hi} 
  E.~Aprile {\it et al.}  [XENON100 Collaboration],
  %``Dark Matter Results from 100 Live Days of XENON100 Data,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 131302 (2011)
  [arXiv:1104.2549 [astro-ph.CO]].


\bibitem{Aprile:2012zx} 
  E.~Aprile [XENON1T Collaboration],
  %``The XENON1T Dark Matter Search Experiment,''
  arXiv:1206.6288 [astro-ph.IM].


  
  \bibitem{Buchmueller:2008qe} 
  O.~Buchmueller, R.~Cavanaugh, A.~De Roeck, J.~R.~Ellis, H.~Flacher, S.~Heinemeyer, G.~Isidori and K.~A.~Olive {\it et al.},
  %``Predictions for Supersymmetric Particle Masses using Indirect Experimental and Cosmological Constraints,''
  JHEP {\bf 0809}, 117 (2008)
  [arXiv:0808.4128 [hep-ph]].
  %%CITATION = ARXIV:0808.4128;%%
  
\bibitem{Buchmueller:2011sw} 
  O.~Buchmueller, R.~Cavanaugh, A.~De Roeck, M.~J.~Dolan, J.~R.~Ellis, H.~Flacher, S.~Heinemeyer and G.~Isidori {\it et al.},
  %``Supersymmetry in Light of 1/fb of LHC Data,''
  Eur.\ Phys.\ J.\ C {\bf 72}, 1878 (2012)
  [arXiv:1110.3568 [hep-ph]].
  %%CITATION = ARXIV:1110.3568;%%
  
    
  \bibitem{Buchmueller:2012hv} 
  O.~Buchmueller, R.~Cavanaugh, M.~Citron, A.~De Roeck, M.~J.~Dolan, J.~R.~Ellis, H.~Flacher and S.~Heinemeyer {\it et al.},
  %``The CMSSM and NUHM1 in Light of 7 TeV LHC, B_s to mu+mu- and XENON100 Data,''
  arXiv:1207.7315 [hep-ph].
  %%CITATION = ARXIV:1207.7315;%%
  
  
  %\cite{Hooper:2012sr}
\bibitem{Hooper:2012sr} 
  D.~Hooper, C.~Kelso and F.~S.~Queiroz,
  ``Stringent and Robust Constraints on the Dark Matter Annihilation Cross Section From the Region of the Galactic Center,''
  arXiv:1209.3015 [astro-ph.HE].
  %%CITATION = ARXIV:1209.3015;%%
  
  %\cite{Ackermann:2011wa}
\bibitem{Ackermann:2011wa} 
  M.~Ackermann {\it et al.}  [Fermi-LAT Collaboration],
  ``Constraining Dark Matter Models from a Combined Analysis of Milky Way Satellites with the Fermi Large Area Telescope,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 241302 (2011)
  [arXiv:1108.3546 [astro-ph.HE]].
  %%CITATION = ARXIV:1108.3546;%%
  
  %\cite{GeringerSameth:2011iw}
\bibitem{GeringerSameth:2011iw} 
  A.~Geringer-Sameth and S.~M.~Koushiappas,
  ``Exclusion of canonical WIMPs by the joint analysis of Milky Way dwarfs with Fermi,''
  Phys.\ Rev.\ Lett.\  {\bf 107}, 241303 (2011)
  [arXiv:1108.2914 [astro-ph.CO]].
  %%CITATION = ARXIV:1108.2914;%%
  
  %\cite{Ackermann:2012rg}
\bibitem{Ackermann:2012rg} 
  T.~F.-M.~Ackermann {\it et al.}  [LAT Collaboration],
  ``Constraints on the Galactic Halo Dark Matter from Fermi-LAT Diffuse Measurements,''
  Astrophys.\ J.\  {\bf 761}, 91 (2012)
  [arXiv:1205.6474 [astro-ph.CO]].
  %%CITATION = ARXIV:1205.6474;%%
  
  \bibitem{Baltz:2008wd} 
  E.~A.~Baltz, B.~Berenji, G.~Bertone, L.~Bergstrom, E.~Bloom, T.~Bringmann, J.~Chiang and J.~Cohen-Tanugi {\it et al.},
 ``Pre-launch estimates for GLAST sensitivity to Dark Matter annihilation signals,''
  JCAP {\bf 0807}, 013 (2008)
  [arXiv:0806.2911 [astro-ph]].
  %%CITATION = ARXIV:0806.2911;%%


\bibitem{Galli:2009zc} 
  S.~Galli, F.~Iocco, G.~Bertone and A.~Melchiorri,
  ``CMB constraints on Dark Matter models with large annihilation cross-section,''
  Phys.\ Rev.\ D {\bf 80}, 023505 (2009)
  [arXiv:0905.0003 [astro-ph.CO]].
  %%CITATION = ARXIV:0905.0003;%%
  
\bibitem{Abramowski:2011hc} 
  A.~Abramowski {\it et al.}  [H.E.S.S. Collaboration],
  ``Search for a Dark Matter annihilation signal from the Galactic Center halo with H.E.S.S,''
  Phys.\ Rev.\ Lett.\  {\bf 106}, 161301 (2011)
  [arXiv:1103.3266 [astro-ph.HE]].
  %%CITATION = ARXIV:1103.3266;%%

\bibitem{Bergstrom:2010gh} 
  L.~Bergstrom, T.~Bringmann and J.~Edsjo,
``Complementarity of direct dark matter detection and indirect detection through gamma-rays,''
  Phys.\ Rev.\ D {\bf 83}, 045024 (2011)
  [arXiv:1011.4514 [hep-ph]].
  %%CITATION = ARXIV:1011.4514;%%

%\cite{Mori:2001dv}
%\bibitem{Mori:2001dv} 
%  K.~Mori, C.~J.~Hailey, E.~A.~Baltz, W.~W.~Craig, M.~Kamionkowski, W.~T.~Serber and P.~Ullio,
  %``A Novel antimatter detector based on x-ray deexcitation of exotic atoms,''
%  Astrophys.\ J.\  {\bf 566}, 604 (2002)
 % [astro-ph/0109463].
  %%CITATION = ASTRO-PH/0109463;%%

\bibitem{Serpico:2011wg} 
  P.~D.~Serpico,
  ``Astrophysical models for the origin of the positron 'excess',''
 Astropart.\ Phys.\  {\bf 39-40}, 2-11 (2012)
  [arXiv:1108.4827].
  %%CITATION = ARXIV:1108.4827;%%
  
%\cite{Weniger:2012tx}
\bibitem{Weniger:2012tx} 
  C.~Weniger,
  ``A Tentative Gamma-Ray Line from Dark Matter Annihilation at the Fermi Large Area Telescope,''
  JCAP {\bf 1208}, 007 (2012)
  [arXiv:1204.2797 [hep-ph]].
  %%CITATION = ARXIV:1204.2797;%%
  
  
\bibitem{Galper:2012fp} 
  A.~M.~Galper, O.~Adriani, R.~L.~Aptekar, I.~V.~Arkhangelskaja, A.~I.~Arkhangelskiy, M.~Boezio, V.~Bonvicini and K.~A.~Boyarchuk {\it et al.},
  ``Status of the GAMMA-400 Project,''
  arXiv:1201.2490 [astro-ph.IM].
  %%CITATION = ARXIV:1201.2490;%%
  
%\cite{Bergstrom:2012vd}
\bibitem{Bergstrom:2012vd} 
  L.~Bergstrom, G.~Bertone, J.~Conrad, C.~Farnier and C.~Weniger,
  ``Investigating Gamma-Ray Lines from Dark Matter with Future Observatories,''
  JCAP {\bf 1211}, 025 (2012)
  [arXiv:1207.6773 [hep-ph]].
  %%CITATION = ARXIV:1207.6773;%%
  
  \bibitem{Hooper:2012ft} 
  D.~Hooper,
  ``The Empirical Case For 10 GeV Dark Matter,''
  arXiv:1201.1303 [astro-ph.CO].
  %%CITATION = ARXIV:1201.1303;%% 
  
  %\cite{Hooper:2012gq}
\bibitem{Hooper:2012gq} 
  D.~Hooper and W.~Xue,
  ``Testing The Light Dark Matter Hypothesis With AMS,''
  arXiv:1210.1220 [astro-ph.HE].
  %%CITATION = ARXIV:1210.1220;%%
  
  \bibitem{Silverwood:2012tp} 
  H.~Silverwood, P.~Scott, M.~Danninger, C.~Savage, J.~Edsjo, J.~Adams, A.~MBrown and K.~Hultqvist,
``Sensitivity of IceCube-DeepCore to neutralino dark matter in the MSSM-25,''
  arXiv:1210.0844 [hep-ph].
  %%CITATION = ARXIV:1210.0844;%%
  
  \bibitem{Koskinen:2011zz} 
  D.~J.~Koskinen,
  %``IceCube-DeepCore-PINGU: Fundamental neutrino and dark matter physics at the South Pole,''
  Mod.\ Phys.\ Lett.\ A {\bf 26}, 2899 (2011).
  %%CITATION = MPLAE,A26,2899;%%


  
{\it Please use the spires labels. 
In case you would like to put more than one reference in the item, please 
add all corresponding spires labels
via `\% bibitem\{BrauJames:2007aa\}', for instance.}
\end{thebibliography}

%\end{document}
% end of file template.tex

